Accelerated Multi-Time-Scale Stochastic Approximation: Optimal Complexity and Applications in Reinforcement Learning and Multi-Agent Games

Multi-time-scale stochastic approximation is an iterative algorithm for finding the fixed point of a set of $N$ coupled operators given their noisy samples. It has been observed that due to the coupling between the decision variables and noisy samples of the operators, the performance of this method decays as $N$ increases. In this work, we develop a new accelerated variant of multi-time-scale stochastic approximation, which significantly improves the convergence rates of its standard counterpart. Our key idea is to introduce auxiliary variables to dynamically estimate the operators from their samples, which are then used to update the decision variables. These auxiliary variables help not only to control the variance of the operator estimates but also to decouple the sampling noise and the decision variables. This allows us to select more aggressive step sizes to achieve an optimal convergence rate. Specifically, under a strong monotonicity condition, we show that for any value of $N$ the $t^{\text{th}}$ iterate of the proposed algorithm converges to the desired solution at a rate $\widetilde{O}(1/t)$ when the operator samples are generated from a single from Markov process trajectory. A second contribution of this work is to demonstrate that the objective of a range of problems in reinforcement learning and multi-agent games can be expressed as a system of fixed-point equations. As such, the proposed approach can be used to design new learning algorithms for solving these problems. We illustrate this observation with numerical simulations in a multi-agent game and show the advantage of the proposed method over the standard multi-time-scale stochastic approximation algorithm.

==> Note.tex <==
Another potential application is \citet{chow2018risk}

==> OldFiles/Sept8_Notation_theta_y/3_analysis.tex <==
\section{Finite-Sample Analysis}
In this section, we establish the finite-sample complexity of \texttt{A-MSA} to the solution of \eqref{eq:obj} when the operators $F_{i}$ have a nested structure. For convenience, we refer to the first and last equations in \eqref{eq:obj} as the highest- and lowest-level problems, respectively, (i.e. $F_N$ is the lowest level problem and $F_1$ is the highest level,) with the level increasing from $N$ to 1. Levels here indicate the order in which the problem can be solved. 
{\color{red}{With some abuse of notation, we denote by $\vtheta_{1:N-1} = \{\theta_1,\cdots,\theta_{N-1}\}$. Given $\vtheta_{1:N-1}$ we use $y_{N}(\vtheta_{1:N-1})$ to denote the solution that solves
\begin{align*}
\widebar{F}_N\Big(\vtheta_{1:N-1},y_{N}(\vtheta_{1:N-1})\Big)=0.
\end{align*}
Similarly, given $\vtheta_{1:N-2}$ we denote by $\{y_{N-1}(\vtheta_{1:N-2}), y_{N}(\vtheta_{1:N-2})\}$ the solution of the lowest two level problems 
\begin{align}
\begin{aligned}
&\widebar{F}_{N-1}\big(\vtheta_{1:N-2},y_{N-1}(\vtheta_{1:N-2}), y_{N}(\vtheta_{1:N-2})\big)=0.\\
&\widebar{F}_{N}\big(\vtheta_{1:N-2},y_{N-1}(\vtheta_{1:N-2}), y_{N}(\vtheta_{1:N-2})\big)=0.
\end{aligned}
\label{eq:two_equations}
\end{align}
To generalize this line of discussion, given any $i\in[2,N]$ we denote by $$\ybf_{i:N}(\vtheta_{1:i-1}) = \{y_{i}(\vtheta_{1:i-1}),\ldots,y_{N}(\vtheta_{1:i-1})\}\quad \text{with}\quad \ybf_{N:N} = y_{N},$$  the solution of
\begin{align*}
\begin{gathered}
\widebar{F}_i\big(\vtheta_{1:i-1}, \ybf_{i:N}(\vtheta_{1:i-1})\big)=0,\quad \forall i = 2,\ldots,N.
\end{gathered}
\end{align*}
When $i=1$ we have $\ybf_{1:N}=\vtheta^{\star}$, which is the optimal solution to \eqref{eq:obj}.

We now introduce the main assumption that drives our analysis, which is the nested strong monotonicity of the operators $\widebar{F}_i$ corresponding to the increasing levels defined above. 
\begin{assump}[Strong Monotonicity]\label{assump:stronglymonotone}
There exists a constant $\delta>0$ such that for all $i=1,\cdots,N-1$ and $\theta_1\in\mathbb{R}^{d_1},\cdots,\theta_{i-1}\in\mathbb{R}^{d_{i-1}}$, $\theta_i,\theta_i' \in \mathbb{R}^{d_i}$
\begin{align*}
    &\Big\langle \widebar{F}_i(\vtheta_{1:i-1},\theta_i,\ybf_{i+1:N}(\vtheta_{1:i-1},\theta_{i}) - \widebar{F}_i(\vtheta_{1:i-1},\theta_i',\ybf_{i+1:N}(\vtheta_{1:i-1},,\theta_{i}'), \theta_i-\theta_i'\Big\rangle \geq\delta \|\theta_i-\theta_i'\|^2.
\end{align*}
\end{assump}}}
%%%%%%%%%%%%%%%%%%%%%%%
The lowest level equation with $F_N$ can be solved independently given any $\{\theta_1,\cdots,\theta_{N-1}\}$ -- we use $y_{N,N}(\{\theta_j\}_{j<N})$ to denote the solution, which satisfies
\begin{align*}
\widebar{F}_N\Big(\theta_1,\cdots,\theta_{N-1},y_{N,N}(\{\theta_j\}_{j<N})\Big)=0.
\end{align*}


The second lowest level equation involving $F_{N-1}$ can be solved for any $\{\theta_1,\cdots,\theta_{N-2}\}$ by finding the optimal solution pair $\big(y_{N\hspace{-1pt}-\hspace{-1pt}1,N\hspace{-1pt}-\hspace{-1pt}1}(\{\theta\}_{j<N\hspace{-1pt}-\hspace{-1pt}1}), y_{N,N}(\{\theta_1,\cdots,\theta_{N-2},y_{N\hspace{-1pt}-\hspace{-1pt}1,N\hspace{-1pt}-\hspace{-1pt}1}(\{\theta\}_{j<N-1})\})\big)$ to the coupled system of two equations
\begin{align}
\begin{aligned}
&\widebar{F}_N\big(\theta_1,\cdots,\theta_{N-2},y_{N-1,N-1}\big(\{\theta_j\}_{j<N-1}\big),y_{N,N}\big(\{\theta_1,\cdots,\theta_{N-2},y_{N-1,N-1}(\{\theta_j\}_{j<N-1})\}\big)\big)=0.\\
&\widebar{F}_{N\hspace{-1pt}-\hspace{-1pt}1}\big(\theta_1,\cdots,\theta_{N-2},y_{N\hspace{-1pt}-\hspace{-1pt}1,N\hspace{-1pt}-\hspace{-1pt}1}\big(\{\theta_j\}_{j<N\hspace{-1pt}-\hspace{-1pt}1}\big),y_{N,N}\big(\{\theta_1,\cdots,\theta_{N\hspace{-1pt}-\hspace{-1pt}2},y_{N-1,N-1}(\{\theta_j\}_{j<N-1})\}\big)\big)=0.
\end{aligned}
\label{eq:two_equations}
\end{align}

To determine $y_{N,N}\big(\{\theta_1,\cdots,\theta_{N-2},y_{N-1,N-1}(\{\theta_j\}_{j<N-1})\}\big)$, we only need to be given $\theta_1$ through $\theta_{N-2}$. 
To simplify the notation, we define \begin{align}
y_{N-1,N}(\{\theta_j\}_{j<N-1})=y_{N,N}(\{\theta_1,\cdots,\theta_{N-2},y_{N-1,N-1}(\{\theta_j\}_{j<N-1})\}),\label{eq:y_transformation:two_equations}
\end{align}
which allows us to re-write \eqref{eq:two_equations} as
\begin{align*}
&\widebar{F}_N\Big(\theta_1,\cdots,\theta_{N-2},y_{N-1,N-1}(\{\theta_j\}_{j<N-1}),y_{N-1,N}(\{\theta_j\}_{j<N-1})\Big)=0.\\
&\widebar{F}_{N-1}\Big(\theta_1,\cdots,\theta_{N-2},y_{N-1,N-1}(\{\theta_j\}_{j<N-1}),y_{N-1,N}(\{\theta_j\}_{j<N-1})\Big)=0.
\end{align*}

To generalize this line of discussion, we define the learning target operator $y_{i,k}:\mathbb{R}^{d_1\times\cdots\times d_{i-1}}\rightarrow\mathbb{R}^{d_k}$ for any $i\in\{2,\cdots,N\}$ and $k\in\{i,\cdots,N\}$ such that given any $\{\theta_j\in\mathbb{R}^{d_j}\}$, $y_{i,k}(\{\theta_j\}_{j<i})$ is the solution to the following system
\begin{align*}
\begin{gathered}
\widebar{F}_i\Big(\theta_1,\cdots,\theta_{i-1}, y_{i,i}(\{\theta_j\}_{j<i}),y_{i,i+1}(\{\theta_j\}_{j<i}),\cdots,y_{i,N}(\{\theta_j\}_{j<i})\Big)=0,\\
\widebar{F}_{i+1}\Big(\theta_1,\cdots,\theta_{i-1}, y_{i,i}(\{\theta_j\}_{j<i}),y_{i,i+1}(\{\theta_j\}_{j<i}),\cdots,y_{i,N}(\{\theta_j\}_{j<i})\Big)=0,\\
\vdots \\
\widebar{F}_{N}\Big(\theta_1,\cdots,\theta_{i-1}, y_{i,i}(\{\theta_j\}_{j<i}),y_{i,i+1}(\{\theta_j\}_{j<i}),\cdots,y_{i,N}(\{\theta_j\}_{j<i})\Big)=0.
\end{gathered}
\end{align*}
For $i=1$, we additionally define $y_{1,k}=\theta_k^{\star}\in\mathbb{R}^{d_k}$, which is the optimal solution to \eqref{eq:obj}.


Conceptually, $y_{i,k}(\{\theta_j\}_{j<i})$ represents the optimal solution of the $k_{\text{th}}$ equation with respect to the $k_{\text{th}}$ variable when $\theta_{1},\cdots,\theta_{i-1}$ are given. 
Generalizing \eqref{eq:y_transformation:two_equations}, we note that for all $i,k$
\begin{align}
y_{i,k}(\{\theta_j\}_{j<i})=y_{k,k}(\{\theta_j\}_{j<i},\{y_{i,i'}(\{\theta_j\}_{j<i})\}_{i'=i,\cdots,k-1}).\label{eq:y_transformation}
\end{align}

We now introduce the most important assumption that drives our analysis, which is the strong monotonicity of each operator $\widebar{F}_i$ with respect to $\theta_i$ structured according to the hierarchy. 
\begin{assump}[Strong Monotonicity]\label{assump:stronglymonotone}
There exists a constant $\delta>0$ such that for all $i=1,\cdots,N$ and $\theta_1\in\mathbb{R}^{d_1},\cdots,\theta_{i-1}\in\mathbb{R}^{d_{i-1}}$, $\theta_i,\theta_i' \in \mathbb{R}^{d_i}$
\begin{align*}
    &\Big\langle \widebar{F}_i(\theta_1,\cdots,\theta_{i-1},\theta_i,y_{i+1,i+1}(\{\theta_j\}_{j\leq i}),\cdots,y_{i+1,N}(\{\theta_j\}_{j\leq i}))\notag\\
    &\hspace{10pt}-\widebar{F}_i(\theta_1,\cdots,\theta_{i-1},\theta_i',y_{i+1,i+1}(\{\theta_j\}_{j< i},\theta_i'),\cdots,y_{i+1,N}(\{\theta_j\}_{j< i},\theta_i')), \theta_i-\theta_i'\Big\rangle \geq\delta \|\theta_i-\theta_i'\|^2.
\end{align*}
\end{assump}
Assumption~\ref{assump:stronglymonotone} states that for any $\theta_1,\cdots,\theta_{i-1}$ the operator $\widebar{F}_i$ is strongly monotone with respect to the $i_{\text{th}}$ decision variable when all lower level decision variables are at the corresponding optimal solutions. When $N=2$, the assumption reduces to the bi-level strong monotonicity assumption commonly made in the literature \citep{doan2022nonlinear,shen2022single,han2024finite} and can be verified to hold in RL applications including the gradient-based TD learning \citep{xu2019two} and distributed TD learning learning\footnote{To model the distributed TD learning in the two-time-scale SA framework, the outer loop equation enforces the consensus among agents whereas in the inner loop each agent learns its local value function.}. The assumption implies that $y_{i,k}(\{\theta_j\}_{j<i})$ is unique for any $\{\theta_j\}_{j<i}$.




\begin{assump}[Lipschitz Continuity and Boundedness]\label{assump:Lipschitz}
There exists positive finite constants $L$ and $B$ such that for all $\vtheta,\vtheta'\in\Omega$
\begin{align}
    % \|\widebar{F}_i(\vtheta)-\widebar{F}_i(\vtheta')\|&\leq L\sum_{j=1}^{N}\|\vtheta_i-\vtheta_i'\|,\quad\forall i,\label{assump:Lipschitz:eq1}\\
    \|F_i(\vtheta,X)-F_i(\vtheta',X)\|&\leq L\sum_{j=1}^{N}\|\theta_i-\theta_i'\|,\quad\forall i,X,\label{assump:Lipschitz:eq1}\\
    \|y_{i,k}(\{\theta_j\}_{j<i})-y_{i,k}(\{\theta_j'\}_{j<i})\|&\leq L\sum_{j=1}^{i-1}\|\theta_j-\theta_j'\|,\quad\forall i,k,\label{assump:Lipschitz:eq2}\\
    \|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})\|&\leq B,\quad\forall i.\label{assump:Lipschitz:eq3}
\end{align}
\end{assump}
Eqs.~\eqref{assump:Lipschitz:eq1} and \eqref{assump:Lipschitz:eq2} are standard Lipschitz continuity assumptions on the operator $F_i$ and learning target \citep{doan2022nonlinear,zeng2024two,shen2022single}. Eq.~\ref{assump:Lipschitz:eq3} assumes that the learning targets are bounded and guarantees algorithm stability in the presence time-varying Markovian noise. This assumption is made in \citet{kaledin2020finite,zeng2024two} which studies solving a system of two equations in the linear and nonlinear settings.
Without any loss of generality, we assume $L\geq\max_{i\in\{1,\cdots,N\},X\in\Xcal}\|F_i(0,X)\|$, which is finite due to the compactness of $\Xcal$. Assumption~\ref{assump:Lipschitz} implies that the operator $F_i$ can be bounded affinely by the decision variable
\begin{align}\label{eq:bounded_F}
\|F_i(\vtheta,X)\|\leq L(\sum_{j=1}^{N}\|\theta_j\|+1),\quad\forall i\in\{1,\cdots,N\},\vtheta\in\Omega.
\end{align}
We use the same constant $L$ in Assumptions~\ref{assump:tv_bound} and \ref{assump:Lipschitz} to simplify the notation.


\noindent\textbf{Convergence Metric.} We quantity the algorithm convergence through the residual variables
\begin{align}
\begin{gathered}
x_i^{[t]}=\theta_i^{[t]}-y_{i,i}(\{\theta_j^{[t]}\}_{j<i}),\qquad \Delta f_i^{[t]}=f_i^{[t]}-\widebar{F}_i(\vtheta^{[t]}).
\end{gathered}\label{eq:residuals}
\end{align}
$x_i^{[t]}$ measures the convergence of decision variable $\theta_i^{[t]}$ by how fast approach the learning target introduced earlier in the section, whereas $\Delta f_i^{[t]}$ measures the convergence of the operator estimation variable $f_i^{[t]}$ to the noiseless $\widebar{F}_i$ evaluated under the latest decision variable. Note that if $x_i^{[t]}=0$ for all $i$, then $\vtheta^{[t]}$ is exactly the (unique) optimal solution $\vtheta^{\star}$.

The step sizes need to be carefully selected for Algorithm~\ref{alg:main} to converge with the best possible rate. In general, $\lambda^{[t]}$ should be larger than $\alpha_i^{[t]}$ for $f_i^{[t]}$ to chase the moving target $\widebar{F}_i(\vtheta^{[t]})$. We choose the step sizes $\lambda^{[t]}$ and $\alpha_i^{[t]}$ to all decay inversely with $t$, differing only by constant multiplicative factors.
\begin{align}
\lambda^{[t]} = \frac{c_{\lambda}}{t+h+1},\quad \alpha_i^{[t]} = \frac{c_i}{t+h+1}.\label{eq:step_sizes}
\end{align}
Here $c_{\lambda}>0$, $c_i>0$, and $h>0$ are constants selected such that for all $i$ and $t$.
\begin{align}
\begin{gathered}
    c_1=\frac{32}{\delta},\quad \lambda^{[t]}\leq1/4, \quad DN^3\tau_t^2\lambda_{t-\tau_t}\leq1/8, \quad\alpha_i^{[t]}\leq\min\{\frac{\delta^2}{80N^8 L^6},\frac{\delta}{40N^5 L^6},\frac{2}{5NL^2},\frac{1}{\delta}\},\\
    \alpha_i^{[t]}\leq\lambda^{[t]}\min\{\frac{1}{8(DN^3+3/\delta+L)},\frac{\delta}{32DN^3},\frac{\delta}{32(\frac{9N^4 L^6}{\delta}+8N^3 L^3)},\frac{16}{\delta}\},\\
    \frac{\alpha_{i-1}^{[t]}}{\alpha_i^{[t]}}\leq\frac{\delta}{16}(\frac{9N^3 L^3}{2}+\frac{4N^6 L^6}{\delta})^{-1},\quad\frac{(\alpha_{i}^{[t]})^2}{\alpha_1^{[t]}}\leq\min\{\frac{\delta^{3/2}}{64N^7},\frac{8}{5N^3 L^3}\}.
\end{gathered}
\label{eq:step_sizes_condition}
\end{align}
We note the parameters satisfying \eqref{eq:step_sizes_condition} always exist and their choices only depend on the structure of operators $F_i$. Here $D$ is a constant as a function of $L$, $B$, $\rho$, and $m$ introduced later.
% in Lemma~\ref{lem:bound_Deltaf}. 


\begin{thm}\label{thm:main}
We define
\begin{align}
V^{[t]}=\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2+\|x_i^{[t]}\|^2].\label{thm:main:Lyapunov}
\end{align}
Under Assumptions~\ref{assump:markov-chain}-\ref{assump:Lipschitz}, the iterates of Algorithm~\ref{alg:main} satisfy for all $t\geq\tau_t$
\begin{align*}
V^{[t+1]}\leq\frac{h^2 V^{[\tau_t]}}{(t+h+1)^2}+\widetilde{\Ocal}\left(\frac{1}{t+1}\right).
\end{align*}
\end{thm}
Theorem~\ref{thm:main} establishes the main result of the work -- it shows that the last iterate of the \texttt{A-MSA} algorithm converges to the unique solution of \eqref{eq:obj} (in the sense of $\sum_{i}\|x_i^{[t]}\|^2$) with a rate of $\widetilde{\Ocal}(1/k)$ under the strong monotonicity condition. 
As the algorithm draws exactly one sample in each iteration, this rate translates to a sample complexity of $\widetilde{\Ocal}(\epsilon^{-1})$ for finding an $\epsilon$-optimal solution. The same complexity has been shown to be achievable by the \texttt{MSA} algorithm under a smoothness assumption on $F_i$ \citep{shen2022single}. We match the rate without requiring this restrictive assumption.
In the absence of the smoothness condition, our rate is order-optimal (up to an logarithm factor) and significantly improves over the best-known rate of \texttt{MSA}, which is $\widetilde{\Ocal}(1/k^{2/3})$ as established in \citet{hong2023two,zeng2024two,han2024finite} when $N=2$. 
Adapting the analysis in these prior works, in Section~\ref{sec:standardSA} we show that the convergence rate of \texttt{MSA} is $\widetilde{\Ocal}(1/k^{1/2})$ when $N=3$ and further deteriorates for $N=4,5,\cdots$. This observation highlights the increasing superiority of our algorithm and analysis over the prior art as $N$ scales up.

\subsection{Proof of Theorem~\ref{thm:main}}

We introduce the following technical lemmas, which set up critical intermediate steps in the proof of Theorem~\ref{thm:main}.
Lemma~\ref{lem:bound_Deltaf} establishes the per-iteration convergence of $\|\Delta f_i^{[t]}\|^2$ in expectation up to (scaled) errors $\sum_{j=1}^{N}\|x_j^{[t]}\|^2$ and $\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2$, whereas Lemma~\ref{lem:bound_x} shows the per-iteration convergence of $\|x_i^{[t]}\|^2$. We note that in \eqref{lem:bound_x:eq1} the terms $\|x_j^{[t]}\|^2$ for $j<i$ and $j>i$ are scaled by different step sizes ($\alpha_j^{[t]}$ versus $\alpha_i^{[t]}$). This subtle difference results from a careful analysis on the coupling effect between $\{\theta_i^{[t]}\}_{i}$ and is key for establishing the optimal complexity. 

\begin{lem}\label{lem:bound_Deltaf}
Under Assumptions~\ref{assump:markov-chain}-\ref{assump:Lipschitz}, the iterates of Algorithm~\ref{alg:main} satisfy for all $t\geq\tau_t$
\begin{align*}
\mathbb{E}[\|\Delta f_i^{[t+1]}\|^2]
&\leq (1-\lambda^{[t]})\mathbb{E}[\|\Delta f_i^{[t]}\|^2]-\frac{\lambda^{[t]}}{4}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]+DN^2\tau_t^2\lambda^{[t]}\lambda^{[t-\tau_t]}\notag\\
&\hspace{20pt}+D N^2 \tau_t^2  (\lambda^{[t]}\lambda^{[t-\tau_t]}+\frac{(\alpha_i^{[t]})^2}{\lambda^{[t]}})\big(\sum_{j=1}^{N}\|x_j^{[t]}\|^2+\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2\big),
\end{align*}
where $D$ is a constant depending only (polynomially) on the structural constants including $L$, $B$, $\rho$, and $m$.
\end{lem}


\begin{lem}\label{lem:bound_x}
Under Assumptions~\ref{assump:markov-chain}-\ref{assump:Lipschitz}, the iterates of Algorithm~\ref{alg:main} satisfy for all $t$
\begin{align}
\|x_i^{[t+1]}\|^2&\leq \|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{4}\|x_i^{[t]}\|^2+\sum_{j=1}^{i-1}\frac{\delta\alpha_j^{[t]}}{8N}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+\left(\frac{9N^3 L^6}{\delta}+8N^2 L^3\right)\alpha_i^{[t]}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2+(\frac{3}{\delta}+L)\alpha_i^{[t]}\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2.\label{lem:bound_x:eq1}
\end{align}
\end{lem}

It is worth noting that if the iterates $\theta_i^{[t]}$ are generated by the \texttt{MSA} algorithm, a per-iteration analysis of $x_i^{[t]}$ similar to Lemma~\ref{lem:bound_x} can be established. We make the analysis and point out the distinctions that allow \texttt{A-MSA} to converge faster later in Section~\ref{sec:standardSA} (Lemma~\ref{lem:conv_x_standardSA}).

We defer the proofs of the lemmas to the appendix but point out that to prove Lemma~\ref{lem:bound_x} the following bound on $\|\theta_i^{[t+1]}-\theta_i^{[t]}\|$ provides an important tool for us to control the stability of the iterates. The implication of Lemma~\ref{lem:Lipschitz} is that the distance $\|\theta_i^{[t+1]}-\theta_i^{[t]}\|$ converges to zero faster than $\Ocal(\alpha_i^{[t]})$ if $\|\Delta f_i^{[t]}\|$ and $\sum_{k=i}^{N}\|x_k^{[t]}\|$ both converge.
\begin{lem}\label{lem:Lipschitz}
Under Assumptions~\ref{assump:markov-chain}-\ref{assump:Lipschitz}, the iterates of Algorithm~\ref{alg:main} satisfy for all $i,t$
\begin{align*}
\|\theta_i^{[t+1]}-\theta_i^{[t]}\|\leq\alpha_i^{[t]}\big(\|\Delta f_i^{[t]}\|+NL^2\sum_{k=i}^{N}\|x_k^{[t]}\|\big).
\end{align*}
\end{lem}



\noindent\textbf{Proof (of Theorem~\ref{thm:main}).}

The proof follows in a straightforward manner by combining the bounds in Lemmas~\ref{lem:bound_Deltaf} and \ref{lem:bound_x} and choosing the correct step sizes. Recall the Lyapunov function \eqref{thm:main:Lyapunov}
\begin{align}
V^{[t+1]}&=\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t+1]}\|^2+\|x_i^{[t+1]}\|^2]\notag\\
&\leq (1-\lambda^{[t]})\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]-\frac{\lambda^{[t]}}{4}\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]+DN^2\tau_t^2\lambda^{[t]}\lambda^{[t-\tau_t]}\notag\\
&\hspace{20pt}+D N^2 \tau_t^2  \sum_{i=1}^N(\lambda^{[t]}\lambda^{[t-\tau_t]}+\frac{(\alpha_i^{[t]})^2}{\lambda^{[t]}})\big(\sum_{j=1}^{N}\|x_j^{[t]}\|^2+\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2\big)\notag\\
&\hspace{20pt}+\sum_{i=1}^{N}\mathbb{E}[\|x_i^{[t]}\|^2]-\sum_{i=1}^{N}\frac{\delta\alpha_i^{[t]}}{4}\mathbb{E}[\|x_i^{[t]}\|^2] +\sum_{i=1}^{N}\sum_{j=1}^{i-1}\frac{\delta\alpha_j^{[t]}}{8N}\mathbb{E}[\|x_j^{[t]}\|^2]\notag\\
&\hspace{20pt}+\sum_{i=1}^{N}\left(\frac{9N^3 L^6}{\delta}+8N^2 L^3\right)\alpha_i^{[t]}\sum_{j=i+1}^{N}\mathbb{E}[\|x_j^{[t]}\|^2]+(\frac{3}{\delta}+L)\sum_{i=1}^{N}\alpha_i^{[t]}\sum_{j=1}^{N}\mathbb{E}[\|\Delta f_j^{[t]}\|^2]\notag\\
&\leq (1-\lambda^{[t]})\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]-\frac{\lambda^{[t]}}{4}\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]+\widetilde{\Ocal}\Big(\frac{1}{(t+1)^2}\Big)\notag\\
&\hspace{20pt}+DN^3\alpha_N^{[t]}\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2] + DN^3 \sum_{i=1}^{N}\frac{(\alpha_i^{[t]})^2}{\lambda^{[t]}}\mathbb{E}[\|x_i^{[t]}\|^2]\notag\\
&\hspace{20pt}+DN^3\tau_t^2\lambda^{[t]}\lambda^{[t-\tau_t]}\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2] + DN^3 \tau_t^2\lambda^{[t]}\lambda^{[t-\tau_t]}\sum_{i=1}^{N}\mathbb{E}[\|x_i^{[t]}\|^2]\notag\\
&\hspace{20pt}+\sum_{i=1}^{N}\mathbb{E}[\|x_i^{[t]}\|^2]-\sum_{i=1}^{N}\frac{\delta\alpha_i^{[t]}}{4}\mathbb{E}[\|x_i^{[t]}\|^2] +\sum_{i=1}^{N}\frac{\delta\alpha_i^{[t]}}{8}\mathbb{E}[\|x_i^{[t]}\|^2]\notag\\
&\hspace{20pt}+\left(\frac{9N^4 L^6}{\delta}+8N^3 L^3\right)\sum_{i=2}^{N}\alpha_{i-1}^{[t]}\mathbb{E}[\|x_i^{[t]}\|^2]+(\frac{3}{\delta}+L)\alpha_N^{[t]}\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]\notag\\
&\leq (1-\lambda^{[t]})\sum_{i=1}^{N}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]+(1-\frac{\delta\alpha_1^{[t]}}{16})\sum_{i=1}^{N}\mathbb{E}[\|x_i^{[t]}\|^2]+\widetilde{\Ocal}\Big(\frac{1}{(t+1)^2}\Big)\notag\\
&\hspace{20pt}-\sum_{i=1}^{N}\left(\frac{\lambda^{[t]}}{8}-(DN^3+\frac{3}{\delta}+L)\alpha_N^{[t]}\right)\mathbb{E}[\|\Delta f_i^{[t]}\|^2]\notag\\
&\hspace{20pt}-\sum_{i=1}^{N}\left(\frac{\delta\alpha_i^{[t]}}{16}-\frac{DN^3 (\alpha_i^{[t]})^2}{\lambda^{[t]}}-\left(\frac{9N^4 L^6}{\delta}+8N^3 L^3\right)\alpha_{i-1}^{[t]}\right)\mathbb{E}[\|x_i^{[t]}\|^2],\label{alg:main:proof_eq1}
\end{align}
where the first inequality plugs in the bounds from Lemmas~\ref{lem:bound_Deltaf} and \ref{lem:bound_x}, and in the last inequality we have artificially introduced $\alpha_0^{[t]}=0$ and used the relation $DN^3\tau_t^2\lambda^{[t-\tau_t]}\leq1/8$. Note that the last two terms of \eqref{alg:main:proof_eq1} are non-positive under the step size condition $\alpha_i^{[t]}\leq\frac{\lambda^{[t]}}{8}(DN^3+\frac{3}{\delta}+L)^{-1}$, $\alpha_i^{[t]}\leq\frac{\delta\lambda^{[t]}}{32DN^3}$, and $\alpha_{[i-1]}^{[t]}\leq\frac{\delta\alpha_i^{[t]}}{32}(\frac{9N^4 L^6}{\delta}+8N^3 L^3)^{-1}$. As a result, we have
\begin{align*}
V^{[t+1]}&\leq\max\{1-\lambda^{[t]},1-\frac{\delta\alpha_1^{[t]}}{16}\}V^{[t]}+\widetilde{\Ocal}\Big(\frac{1}{(t+1)^2}\Big)\notag\\
&\leq(1-\frac{\delta\alpha_1^{[t]}}{16})V^{[t]}+\widetilde{\Ocal}\Big(\frac{1}{(t+1)^2}\Big)\notag\\
&\leq (1-\frac{2}{t+h+1})V^{[t]}+\widetilde{\Ocal}\Big(\frac{1}{(t+1)^2}\Big),
\end{align*}
due to $\alpha_{1}^{[t]}\leq\frac{16\lambda^{[t]}}{\delta}$ and $c_1=\frac{32}{\delta}$.

Multiplying by $(t+h+1)^2$ on both sides, we have
\begin{align*}
(t+h+1)^2 V^{[t+1]}&\leq(t+h+1)(t+h-1)V^{[t]}+\widetilde{\Ocal}(1)\notag\\
&\leq (t+h)^2 V^{[t]}+\widetilde{\Ocal}(1)\notag\\
&\leq h^2 V^{[\tau_t]}+\widetilde{\Ocal}(t+1).
\end{align*}


Dividing by $(t+h+1)^2$ now, we have
\begin{align*}
    V^{[t+1]}\leq\frac{h^2 V^{[\tau_t]}}{(t+h+1)^2}+\widetilde{\Ocal}\left(\frac{1}{t+1}\right).
\end{align*}

\qed

==> OldFiles/Sept8_Notation_theta_y/4_standardSA.tex <==
\subsection{Standard Multi-Time-Scale Stochastic Approximation}\label{sec:standardSA}

In this section, we present the finite-time complexity of the \texttt{MSA} algorithm derived using the techniques in \citet{hong2023two,zeng2024two}, with the purpose of highlighting its gap from the optimal $\widetilde{\Ocal}(1/t)$ rate established in Theorem~\ref{thm:main}. We start with the case of three equations ($N=3$), where the objective is to solve
\begin{align*}
\begin{array}{c}
     \widebar{F}_1(\theta_1,\theta_2,\theta_3)=0, \\
     \widebar{F}_2(\theta_1,\theta_2,\theta_3)=0, \\
     \widebar{F}_3(\theta_1,\theta_2,\theta_3)=0.
\end{array}
\end{align*}



Recall the update rule of \texttt{MSA} in \eqref{alg:update_standardSA}. 
For simplicity, we assume (just in this section) that that stationary distribution $\mu_{\vtheta}=\mu$ is independent of $\vtheta$ and that each $X^{[t]}$ is an i.i.d. sample from $\mu$. 


We additionally assume that $F_i$ has uniformly bounded energy as follows. Note that this is not a necessary assumption but considered just to simplify the analysis of \texttt{MSA}. Also note that we do not make this assumption in the analysis of the proposed \texttt{A-MSA} algorithm.


\begin{assump}\label{assump:bounded}
There exists a constant $D>0$ such that for all $i=1,2,3$, $\theta_i \in \mathbb{R}^{d_i}$, and $X\in\Xcal$
\begin{align*}
\| F_i(\theta_1,\theta_2,\theta_3,X)\|\leq D.
\end{align*}
\end{assump}


We measure the convergence by $x_i^{[t]}$, which is the same as the metric \eqref{eq:residuals} used for analyzing \texttt{A-MSA}.
\begin{align*}
x_i^{[t]}=\theta_i^{[t]}-y_{i,i}(\{\theta_j^{[t]}\}_{j<i}).
\end{align*}


We establish the per-iteration convergence of $x_i^{t}$ in the lemma below. We defer its proof to Appendix~\ref{sec:proof_lem:conv_x_standardSA}. 
\begin{lem}\label{lem:conv_x_standardSA}
We artificially define $\alpha_0^{[t]}=0$ for all $t$.
Under Assumptions~\ref{assump:stronglymonotone}-\ref{assump:bounded}, the iterates of the \texttt{MSA} algorithm in \eqref{alg:update_standardSA} satisfy for all $t\geq0$
\begin{align*}
\mathbb{E}[\|x_i^{[t+1]}\|^2]
&\leq \mathbb{E}[\|x_i^{[t]}\|^2]-\frac{\delta\alpha_i^{[t]}}{4}\mathbb{E}[\|x_i^{[t]}\|^2]+\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\mathbb{E}[\|x_j^{[t]}\|^2]\\
&\hspace{120pt}+8N^2 L^2 D^2 (\alpha_{i}^{[t]})^2+\frac{N^2 L^2 D^2 (\alpha_{i-1}^{[t]})^2}{\delta\alpha_i^{[t]}}.
\end{align*}
\end{lem}

It is worth noting that Lemma~\ref{lem:conv_x_standardSA} holds for any $N$. We apply this lemma to the case $N=3$ and consider the Lyapunov function 
\begin{align}
V^{[t]}=\mathbb{E}[\|x_1^{[t]}\|^2+v_2^{[t]}\|x_2^{[t]}\|^2+v_3^{[t]}\|x_3^{[t]}\|^2],\label{eq:standardSA_lyapunov}
\end{align}
where $v_2^{[t]}=\frac{1728 L^6\alpha_1^{[t]}}{\delta^2\alpha_2^{[t]}}$ and $v_3^{[t]}=\frac{8\alpha_1^{[t]}}{\delta\alpha_3^{[t]}}(\frac{216 L^6}{\delta}+\frac{373248L^{12}}{\delta^3})$.

\begin{thm}\label{thm:standardSA}
Let the step sizes be
\begin{align}
\alpha_1^{[t]}=\frac{c_1}{t+h+1},\quad \alpha_2^{[t]}=\frac{c_2}{(t+h+1)^{3/4}},\quad \alpha_2^{[t]}=\frac{c_3}{(t+h+1)^{1/2}},\label{thm:standardSA:step_size}
\end{align}
with proper choices of the constants $c_1,c_2,c_3$, and $h$.
Under Assumptions~\ref{assump:stronglymonotone}-\ref{assump:bounded}, the iterates of the \texttt{MSA} algorithm in \eqref{alg:update_standardSA} with i.i.d. samples $X^{[t]}\sim\mu$ satisfy for all $t\geq0$
\begin{align*}
V^{[t+1]}\leq\Ocal\left(\frac{V^{[0]}}{(t+\tau+1)^{1/2}}\right).
\end{align*}
\end{thm}

\textbf{Proof.}

With $N=3$, Lemma~\ref{lem:conv_x_standardSA} implies
\begin{align*}
\mathbb{E}[\|x_1^{[t+1]}\|^2]&\hspace{-2pt}\leq\hspace{-2pt} (1\hspace{-2pt}-\hspace{-2pt}\frac{\delta\alpha_1^{[t]}}{4})\mathbb{E}[\|x_1^{[t]}\|^2]+\frac{216 L^6\alpha_1^{[t]}}{\delta}\mathbb{E}[\|x_2^{[t]}\|^2+\|x_3^{[t]}\|^2]+72 L^2 D^2 (\alpha_1^{[t]})^2,\\
\mathbb{E}[\|x_2^{[t+1]}\|^2]&\hspace{-2pt}\leq\hspace{-2pt} (1\hspace{-2pt}-\hspace{-2pt}\frac{\delta\alpha_2^{[t]}}{4})\mathbb{E}[\|x_2^{[t]}\|^2]\hspace{-2pt}+\hspace{-2pt}\frac{216 L^6\alpha_2^{[t]}}{\delta}\mathbb{E}[\|x_3^{[t]}\|^2]\hspace{-2pt}+\hspace{-2pt}72 L^2 D^2 (\alpha_{2}^{[t]})^2\hspace{-2pt}+\hspace{-2pt}\frac{9 L^2 D^2 (\alpha_1^{[t]})^2}{\delta\alpha_2^{[t]}},\\
\mathbb{E}[\|x_3^{[t+1]}\|^2]&\hspace{-2pt}\leq\hspace{-2pt} (1\hspace{-2pt}-\hspace{-2pt}\frac{\delta\alpha_3^{[t]}}{4})\mathbb{E}[\|x_3^{[t]}\|^2]+72 L^2 D^2 (\alpha_3^{[t]})^2+\frac{9 L^2 D^2 (\alpha_2^{[t]})^2}{\delta\alpha_3^{[t]}}.
\end{align*}


Recall the Lyapunov function 
$V^{[t]}=\mathbb{E}[\|x_1^{[t]}\|^2+v_2^{[t]}\|x_2^{[t]}\|^2+v_3^{[t]}\|x_3^{[t]}\|^2]$. Note that $v_2^{[t+1]}\leq v_2^{[t]}$ and $v_3^{[t+1]}\leq v_3^{[t]}$ since $\alpha_1^{[t]}$ decays faster than $\alpha_2^{[t]},\alpha_3^{[t]}$. We have
\begin{align}
V^{[t+1]}&=\mathbb{E}[\|x_1^{[t+1]}\|^2+v_2^{[t+1]}\|x_2^{[t+1]}\|^2+v_3^{[t+1]}\|x_3^{[t+1]}\|^2]\notag\\
&\leq \mathbb{E}[\|x_1^{[t+1]}\|^2+v_2^{[t]}\|x_2^{[t+1]}\|^2+v_3^{[t]}\|x_3^{[t+1]}\|^2]\notag\\
&\leq(1-\frac{\delta\alpha_1^{[t]}}{4})\mathbb{E}[\|x_1^{[t]}\|^2]+\frac{216 L^6\alpha_1^{[t]}}{\delta}\mathbb{E}[\|x_2^{[t]}\|^2+\|x_3^{[t]}\|^2]+72 L^2 D^2 (\alpha_{1}^{[t]})^2\notag\\
&\hspace{20pt}+v_2^{[t]}(1-\frac{\delta\alpha_2^{[t]}}{4})\mathbb{E}[\|x_2^{[t]}\|^2]+\frac{216 L^6\alpha_2^{[t]}v_2^{[t]}}{\delta}\mathbb{E}[\|x_3^{[t]}\|^2]+72 L^2 D^2 (\alpha_{2}^{[t]})^2 v_2^{[t]}\notag\\
&\hspace{20pt}+\frac{9 L^2 D^2 (\alpha_1^{[t]})^2 v_2^{[t]}}{\delta\alpha_2^{[t]}}+v_3^{[t]}(1-\frac{\delta\alpha_3^{[t]}}{4})\mathbb{E}[\|x_3^{[t]}\|^2]\notag\\
&\hspace{20pt}+72 L^2 D^2 (\alpha_3^{[t]})^2 v_3^{[t]}+\frac{9 L^2 D^2 (\alpha_2^{[t]})^2 v_3^{[t]}}{\delta\alpha_3^{[t]}}\notag\\
&=(1-\frac{\delta\alpha_1^{[t]}}{4})\mathbb{E}[\|x_1^{[t]}\|^2+v_2^{[t]}\|x_2^{[t]}\|^2+v_3^{[t]}\|x_3^{[t]}\|^2]+72 L^2 D^2 (\alpha_{1}^{[t]})^2\notag\\
&\hspace{20pt}+\frac{124416 L^8 D^2 \alpha_{1}^{[t]}\alpha_{2}^{[t]}}{\delta^2}+\frac{15552 L^8 D^2 (\alpha_1^{[t]})^3}{\delta^3(\alpha_2^{[t]})^2}\notag\\
&\hspace{20pt}+\left(\frac{572L^2 D^2\alpha_1^{[t]}\alpha_3^{[t]}}{\delta}+\frac{9L^2 D^2 \alpha_1^{[t]}(\alpha_2^{[t]})^2}{\delta^2(\alpha_3^{[t]})^2}\right)(\frac{216 L^6}{\delta}+\frac{373248L^{12}}{\delta^3})\notag\\
&\hspace{20pt}+(\frac{\delta \alpha_1^{[t]} v_2^{[t]}}{4}-\frac{\delta \alpha_2^{[t]} v_2^{[t]}}{4}+\frac{216 L^6\alpha_1^{[t]}}{\delta})\mathbb{E}[\|x_2^{[t]}\|^2]\notag\\
&\hspace{20pt}+(\frac{\delta \alpha_1^{[t]} v_3^{[t]}}{4}-\frac{\delta \alpha_3^{[t]} v_3^{[t]}}{4}+\frac{216 L^6\alpha_1^{[t]}}{\delta}+\frac{216 L^6\alpha_2^{[t]}v_2^{[t]}}{\delta})\mathbb{E}[\|x_3^{[t]}\|^2]\notag\\
&\leq(1-\frac{\delta\alpha_1^{[t]}}{4})V^{[t]}+72 L^2 D^2 (\alpha_{1}^{[t]})^2+\frac{124416 L^8 D^2 \alpha_{1}^{[t]}\alpha_{2}^{[t]}}{\delta^2}+\frac{15552 L^8 D^2 (\alpha_1^{[t]})^3}{\delta^3(\alpha_2^{[t]})^2}\notag\\
&\hspace{20pt}+\left(\frac{572L^2 D^2\alpha_1^{[t]}\alpha_3^{[t]}}{\delta}+\frac{9L^2 D^2 \alpha_1^{[t]}(\alpha_2^{[t]})^2}{\delta^2(\alpha_3^{[t]})^2}\right)(\frac{216 L^6}{\delta}+\frac{373248L^{12}}{\delta^3}),\label{thm:standardSA:proof_eq1}
\end{align}
where the last inequality is a result of 
\begin{align*}
&\frac{\delta \alpha_1^{[t]} v_2^{[t]}}{4}-\frac{\delta \alpha_2^{[t]} v_2^{[t]}}{4}+\frac{216 L^6\alpha_1^{[t]}}{\delta}=\frac{\delta \alpha_1^{[t]} v_2^{[t]}}{4}-\frac{\delta \alpha_2^{[t]} v_2^{[t]}}{8}\leq0,\\
&\frac{\delta \alpha_1^{[t]} v_3^{[t]}}{4}-\frac{\delta \alpha_3^{[t]} v_3^{[t]}}{4}+\frac{216 L^6\alpha_1^{[t]}}{\delta}+\frac{216 L^6\alpha_2^{[t]}v_2^{[t]}}{\delta}\\
&=\frac{\delta \alpha_1^{[t]} v_3^{[t]}}{4}-\frac{\delta \alpha_3^{[t]} v_3^{[t]}}{4}+\frac{216 L^6\alpha_1^{[t]}}{\delta}+\frac{373248L^{12}\alpha_1^{[t]}}{\delta^3}=\frac{\delta \alpha_1^{[t]} v_3^{[t]}}{4}-\frac{\delta \alpha_3^{[t]} v_3^{[t]}}{8}\leq0,
\end{align*}
following from the step size condition $\alpha_1^{[t]}\leq\frac{\alpha_2^{[t]}}{2}\leq \frac{\alpha_3^{[t]}}{2}$.

Under the step size rule \eqref{thm:standardSA:step_size} with $c_1\geq\frac{8}{\delta}$, it can be easily derived that
\begin{align*}
V^{[t+1]}&\leq(1-\frac{2}{t+h+1})V^{[t]}+\Ocal(1/t^{3/2}).
\end{align*}

Then, following the standard argument, we have
\begin{align*}
V^{[t+1]}\leq\Ocal(\frac{V^{[0]}}{(t+h+1)^{1/2}}).
\end{align*}

\qed


We now discuss how Theorem~\ref{thm:standardSA} can be extended to more than three equations and what the expected convergence rate should be. 
When $N=2$, \citet{zeng2024two} shows that the convergence rate is on the order of (up to a logarithm factor)
\begin{align}
\max\Big\{\alpha_1^{[t]},\alpha_2^{[t]},\Big(\frac{\alpha_1^{[t]}}{\alpha_2^{[t]}}\Big)^2\Big\}.\label{eq:convrate_stepsize_N2}
\end{align}
To optimize \eqref{eq:convrate_stepsize_N2} the step sizes should be selected as $\alpha_1^{[t]}\sim\frac{1}{k}, \alpha_2^{[t]}\sim\frac{1}{k^{2/3}}$, which leads to a convergence rate of $\widetilde{\Ocal}(t^{-2/3})$. 

When $N=3$, the convergence rate is on the order of
\begin{align*}
\max\Big\{\alpha_1^{[t]},\alpha_2^{[t]},\alpha_3^{[t]},\Big(\frac{\alpha_1^{[t]}}{\alpha_2^{[t]}}\Big)^2,\Big(\frac{\alpha_2^{[t]}}{\alpha_3^{[t]}}\Big)^2\Big\}.
\end{align*}
which dictates the choice of step sizes in \eqref{thm:standardSA:step_size}.

For general $N$, we can expect the convergence rate to be
\begin{align}
\max\Big\{\alpha_1^{[t]},\cdots,\alpha_N^{[t]},\Big(\frac{\alpha_1^{[t]}}{\alpha_2^{[t]}}\Big)^2,\cdots,\Big(\frac{\alpha_{N-1}^{[t]}}{\alpha_N^{[t]}}\Big)^2\Big\}.\label{eq:convrate_stepsize_N}
\end{align}
It is straightforward to see that the optimal decay rate of \eqref{eq:convrate_stepsize_N} is $\widetilde{\Ocal}(t^{-2/(N+1)})$. 




\subsection{Reflecting on Faster Convergence of \texttt{A-MSA}}\label{sec:comparison}

Lemmas~\ref{lem:bound_x} and \ref{lem:conv_x_standardSA} establish critical per-iteration convergence bounds on the errors in the decision variable for \texttt{A-MSA} and \texttt{MSA}, respectively. In this section, we contrast corresponding terms in the bounds to pinpoint the advantage of Lemma~\ref{lem:bound_x} over Lemma~\ref{lem:conv_x_standardSA}. In the analysis of $\|x_i^{[t+1]}\|^2$ under the two algorithms, the common/comparable terms include the following:
\begin{itemize}
\item $\|y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t]}\}_{j<i})\|$ arises from the shift in learning target $y_{i,i}(\{\theta_j^{[t]}\}_{j<i})$ across iterations and appears in the analysis of both Lemma~\ref{lem:bound_x} and Lemma~\ref{lem:conv_x_standardSA}. Due to the Lipschitz continuity of $y_{i,i}$ imposed in Assumption~\ref{assump:Lipschitz}, controlling this term essentially requires handling
\begin{align}
\sum_{j=1}^{i-1}\|\theta_j^{[t+1]}-\theta_j^{[t]}\|.\label{eq:contrast_eq1}
\end{align}

Under the \texttt{MSA} algorithm, there currently exists no better way of bounding \eqref{eq:contrast_eq1} than
using $\sum_{j=1}^{i-1}\alpha_j^{[t]}\|F_i(\vtheta^{[t]},X^{[t]})\|$. As $\|F_i(\vtheta^{[t]},X^{[t]})\|$ is on the order of a constant even when $\vtheta^{[t]}$ approaches the optimal solution (due to the random sample $X^{[t]}$), the bound eventually becomes $\Ocal(\alpha_{i-1})$.

In comparison, under \texttt{A-MSA}, we can control \eqref{eq:contrast_eq1} with Lemma~\ref{lem:Lipschitz} and show 
\begin{align}
    \sum_{j=1}^{i-1}\|\theta_j^{[t+1]}-\theta_j^{[t]}\|\leq\Ocal\Big(\sum_{j=1}^{i-1}\alpha_j^{[t]}\|\Delta f_j^{[t]}\|+\sum_{j=1}^{i-1}\alpha_j^{[t]}\|x_j^{[t]}\|+\alpha_{i-1}^{[t]}\sum_{j=i}^{N}\|x_j^{[t]}\|\Big).\label{eq:contrast_eq2}
\end{align}
Since $\|\Delta f_j^{[t]}\|$ and $\|x_j^{[t]}\|$ themselves decay to zero as the iterations proceed, the convergence rate of \eqref{eq:contrast_eq2} is much faster than $\Ocal(\alpha_{i-1})$.

\noindent\textbf{Takeaway:} 
Our objective is to solve a highly coupled system \eqref{eq:obj}.
The discussion above highlights how the \texttt{A-MSA} algorithm effectively decouples the decision variables, in the sense that the inaccuracy of upper-level variables has a reduced effect on the analysis of lower-level ones. Being able to decoupled the decision variable updates is crucial as it allows us to choose $\alpha_i^{[t]}$ across $i$ in a more independent manner.


\item $\|\Delta f_i^{[t]}\|^2=\|f_i^{[t]}-\widebar{F}_i(\vtheta^{[t]})\|^2$ is an error appearing in the proof of Lemma~\ref{lem:bound_x} for \texttt{A-MSA}, whereas $\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2$ is the comparable term that shows up in the proof of Lemma~\ref{lem:conv_x_standardSA} for \texttt{MSA}. They capture the variance in the estimation of $\widebar{F}_i(\vtheta^{[t]})$. In the case of \texttt{MSA}, $\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2$ does not decay to zero (again due to the randomness in $X^{[t]}$), which eventually becomes a bottleneck in achieving the optimal rate. In contrast, $\|\Delta f_i^{[t]}\|^2$ under \texttt{A-MSA} can be expected to converge to zero (under a careful analysis).

\noindent\textbf{Takeaway:} 
Compared to \texttt{MSA}, \texttt{A-MSA} provides a low-variance estimate of $\widebar{F}_i(\vtheta^{[t]})$. The variance decaying sufficiently fast is another key driver of the overall improved complexity.

\end{itemize}

\begin{remark}
At the end of the section, we point out an important additional advantage of the analysis of \texttt{A-MSA} over that of \texttt{MSA}. Observe that the Lyapunov function \eqref{eq:standardSA_lyapunov} considered in Theorem~\ref{thm:standardSA} weights the lower-level residuals $x_2^{[t]}$ and $x_3^{[t]}$ by $v_2^{[t]}$ and $v_3^{[t]}$. The weights have been carefully chosen to ensure the proper cancellation of errors across different levels. Choosing such weights, however, requires non-trivial efforts and can be inconvenient as $N$ goes up. 

In addition, we note that the weights $v_2^{[t]}$ and $v_3^{[t]}$ themselves are decaying sequences. Theorem~\ref{thm:standardSA} shows that $V^{[t]}$ decays with rate $\widetilde{\Ocal}(t^{-1/2})$, which only implies $\mathbb{E}[\|x_2^{[t]}\|^2]\leq\widetilde{\Ocal}(t^{-1/4})$ and $\mathbb{E}[\|x_3^{[t]}\|^2]\leq\widetilde{\Ocal}(1)$. In other words, the guaranteed convergence rate of lower-level variables does not match that of the highest level variable and may even be meaningless.
In contrast, the Lyapunov function \eqref{thm:main:Lyapunov} for the analysis of \texttt{A-MSA} simply combines $\|x_i^{[t]}\|^2$ over all levels without additional weights. As a result, the decision variables at all level are guaranteed to converge at $\widetilde{\Ocal}(t^{-1})$.
\end{remark}




==> OldFiles/Sept8_Notation_theta_y/Proof_Lemmas.tex <==
\section{Proof of Technical Lemmas}\label{sec:proof_lemmas}



\subsection{Proof of Lemma~\ref{lem:bound_Deltaf}}


\begin{lem}\label{lem:Markovian_crossterm}
For any $t\geq\tau_t$ we have
\begin{align*}
\mathbb{E}[\langle\Delta f_i^{[t]},F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle]\leq N^2 C_{\tau}\tau_t^2\lambda^{[t-\tau_t]}\Big(\sum_{j=1}^{N}\|x_j^{[t]}\|^2+\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2+1\Big),
\end{align*}
where $C_{\tau}$ is a positive, bounded scalar depending only on the structural constants including $L$, $B$, $\rho$, and $m$.
\end{lem}



We derive a frequently used inequality in the proofs of Lemma~\ref{lem:bound_Deltaf} and \ref{lem:Markovian_crossterm} as a result of \eqref{eq:bounded_F}. For any $X$, we have
\begin{align}
\|F_i(\vtheta^{[t]},X)\|&\leq L(\sum_{j=1}^N\|\theta_j^{[t]}\|+1)\notag\\
&\leq L+L\sum_{j=1}^N\|\theta_j^{[t]}-y_{j,j}(\{\theta_k^{[t]}\}_{k<j})\|+L\sum_{j=1}^N\|y_{j,j}(\{\theta_k^{[t]}\}_{k<j})\|\notag\\
&\leq (NB+1)L+L\sum_{j=1}^{N}\|x_j^{[t]}\|,
\label{lem:bound_Deltaf:boundedF}
\end{align}
where the last inequality follows from the boundedness condition in Assumption~\ref{assump:Lipschitz} and the definition of $x_j^{[t]}$ in \eqref{eq:residuals}.


By the update rule in \eqref{eq:update_auxiliary}, we have
\begin{align*}
    \Delta f_i^{[t+1]}&=f_i^{[t+1]}-\widebar{F}_i(\vtheta^{[t+1]})\notag\\
    &=(1-\lambda^{[t]})f_i^{[t]}+\lambda^{[t]}F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\notag\\
    &=(1-\lambda^{[t]})f_i^{[t]}+\lambda^{[t]}\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})+\lambda^{[t]}\left(F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\right)\notag\\
    &=(1-\lambda^{[t]})\Delta f_i^{[t]}+\left(\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\right)+\lambda^{[t]}\left(F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\right).
\end{align*}

This leads to
\begin{align}
&\|\Delta f_i^{[t+1]}\|^2\notag\\
&=(1-\lambda^{[t]})^2\|\Delta f_i^{[t]}\|^2+\|\left(\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\right)+\lambda^{[t]}\left(F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\right)\|^2\notag\\
&\hspace{20pt}+2(1-\lambda^{[t]})\langle\Delta f_i^{[t]},\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\rangle\notag\\
&\hspace{20pt}+2\lambda^{[t]}(1-\lambda^{[t]})\langle\Delta f_i^{[t]},F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle\notag\\
&\leq(1-\lambda^{[t]})^2\|\Delta f_i^{[t]}\|^2+2\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\|^2+2(\lambda^{[t]})^2\|\widebar{F}_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2\notag\\
&\hspace{20pt}+\frac{\lambda^{[t]}}{2}\|\Delta f_i^{[t]}\|^2+\frac{2}{\lambda^{[t]}}\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\|^2\notag\\
&\hspace{20pt}+2\lambda^{[t]}(1-\lambda^{[t]})\langle\Delta f_i^{[t]},F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle\notag\\
&\leq(1-\lambda^{[t]})\|\Delta f_i^{[t]}\|^2-\frac{\lambda^{[t]}}{4}\|\Delta f_i^{[t]}\|^2+2(\lambda^{[t]})^2\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2\notag\\
&\hspace{20pt}+\frac{4}{\lambda^{[t]}}\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\|^2+2\lambda^{[t]}(1-\lambda^{[t]})\langle\Delta f_i^{[t]},F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle,
\label{lem:bound_Deltaf:proof_eq1}
\end{align}
where the last inequality follows from $\lambda^{[t]}\leq1/4\leq 1$. 

Note that the third term on the right hand side of \eqref{lem:bound_Deltaf:proof_eq1} is bounded due to \eqref{lem:bound_Deltaf:boundedF}
\begin{align}
\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2 &\leq  2\|F_i(\vtheta^{[t]},X^{[t]})\|+2\|\widebar{F}_i(\vtheta^{[t]})\|^2\notag\\
&\leq 4\Big((NB+1)L+L\sum_{j=1}^{N}\|x_j^{[t]}\|\Big)^2\notag\\
&\leq 8L^2\big(N\sum_{j=1}^N\|x_j^{[t]}\|^2+(NB+1)^2\big).
\label{lem:bound_Deltaf:proof_eq1.1}
\end{align}


For the fourth term of \eqref{lem:bound_Deltaf:proof_eq1}, we have from Lemma~\ref{lem:Lipschitz} and the Lipschitz continuity of $\widebar{F}_i$ 
\begin{align}
\mathbb{E}[\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\|^2]&\leq L^2\sum_{j=1}^{N}\mathbb{E}[\|\theta_j^{[t]}-\theta_j^{[t+1]}\|^2]\notag\\
&\leq L^2(\alpha_i^{[t]})^2\sum_{j=1}^{N}\mathbb{E}[\left(\|\Delta f_j^{[t]}\|+NL^2\sum_{k=j}^{N}\|x_k^{[t]}\|\right)^2]\notag\\
&\leq 2L^2(\alpha_i^{[t]})^2\sum_{j=1}^{N}\mathbb{E}[\|\Delta f_j^{[t]}\|^2]+2NL^4(\alpha_i^{[t]})^2\sum_{j=1}^{N}\sum_{k=j}^{N}\mathbb{E}[\|x_k^{[t]}\|^2]\notag\\
&\leq 2L^2(\alpha_i^{[t]})^2\sum_{j=1}^{N}\mathbb{E}[\|\Delta f_j^{[t]}\|^2]+2N^2L^4(\alpha_i^{[t]})^2\sum_{j=1}^{N}\mathbb{E}[\|x_j^{[t]}\|^2].
\end{align}


The last term of \eqref{lem:bound_Deltaf:proof_eq1} is bound in expectation due to Lemma~\ref{lem:Markovian_crossterm}
\begin{align}
\mathbb{E}[\langle\Delta f_i^{[t]},F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle]\leq N^2 C_{\tau}\tau_t^2\lambda^{[t-\tau_t]}\Big(\sum_{j=1}^{N}\|x_j^{[t]}\|^2+\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2+1\Big).
\label{lem:bound_Deltaf:proof_eq1.2}
\end{align}

Combining \eqref{lem:bound_Deltaf:proof_eq1.1}-\eqref{lem:bound_Deltaf:proof_eq1.2} with
\eqref{lem:bound_Deltaf:proof_eq1},
\begin{align}
    &\mathbb{E}[\|\Delta f_i^{[t+1]}\|^2]\notag\\
    &\leq (1-\lambda^{[t]})\mathbb{E}[\|\Delta f_i^{[t]}\|^2]-\frac{\lambda^{[t]}}{4}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]+2(\lambda^{[t]})^2\mathbb{E}[\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2]\notag\\
    &\hspace{20pt}+\frac{4}{\lambda^{[t]}}\mathbb{E}[\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t+1]})\|^2]+2\lambda^{[t]}(1-\lambda^{[t]})\mathbb{E}[\langle\Delta f_i^{[t]},F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle]\notag\\
    &\leq (1-\lambda^{[t]})\mathbb{E}[\|\Delta f_i^{[t]}\|^2]-\frac{\lambda^{[t]}}{4}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]+8L^2(\lambda^{[t]})^2\big(N\sum_{j=1}^N\|x_j^{[t]}\|^2+(NB+1)^2\big)\notag\\
    &\hspace{20pt}+\frac{8L^2(\alpha_i^{[t]})^2}{\lambda^{[t]}}\sum_{j=1}^{N}\mathbb{E}[\|\Delta f_j^{[t]}\|^2] + \frac{8N^2 L^4(\alpha_i^{[t]})^2}{\lambda^{[t]}}\sum_{j=1}^{N}\mathbb{E}[\|x_j^{[t]}\|^2]\notag\\
    &\hspace{20pt}+N^2 C_{\tau}\tau_t^2\lambda^{[t]}\lambda^{[t-\tau_t]}(\sum_{j=1}^{N}\|x_j^{[t]}\|^2+\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2+1)\notag\\
    &\leq (1-\lambda^{[t]})\mathbb{E}[\|\Delta f_i^{[t]}\|^2]-\frac{\lambda^{[t]}}{4}\mathbb{E}[\|\Delta f_i^{[t]}\|^2]+DN^2\tau_t^2\lambda^{[t]}\lambda^{[t-\tau_t]}\notag\\
    &\hspace{20pt}+D N^2 \tau_t^2  (\lambda^{[t]}\lambda^{[t-\tau_t]}+\frac{(\alpha_i^{[t]})^2}{\lambda^{[t]}})\big(\sum_{j=1}^{N}\|x_j^{[t]}\|^2+\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2\big),
\end{align}
where $D$ is a finite constant depending only on $L$, $B$, and $C_{\tau}$.


\qed



\subsection{Proof of Lemma~\ref{lem:bound_x}}

By the update rule in \eqref{alg:update_decision}, we have
\begin{align*}
x_i^{[t+1]}&=\theta_{i}^{[t+1]}-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\notag\\
&=\theta_{i}^{[t]}-\alpha_i^{[t]}f_i^{[t]}-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\notag\\
&=x_i^{[t]}-\alpha_i^{[t]}f_i^{[t]}+\left(y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\right)\notag\\
&=x_i^{[t]}-\alpha_i^{[t]} \widebar{F}_i(\vtheta^{[t]})-\alpha_i^{[t]}\Delta f_i^{[t]}+\left(y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\right)\notag\\
% &=x_i^{[t]}-\alpha_i^{[t]} F_i(\{\theta_j^{[t]}\}_{j\leq i},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k=i+1,\cdots,N})\notag\\
% &\hspace{20pt}+\alpha_i^{[t]} \left(\widebar{F}_i(\{\theta_j^{[t]}\}_{j\leq i},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k=i+1,\cdots,N})-\widebar{F}_i(\vtheta^{[t]})\right)\notag\\
% &\hspace{20pt}-\alpha_i^{[t]}\Delta f_i^{[t]}+\left(y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\right).
\end{align*}

Taking the norm leads to
\begin{align}
&\|x_i^{[t+1]}\|^2 \notag\\
& \leq \underbrace{\|x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]})\|^2}_{T_1} + (\alpha_i^{[t]})^2\|\Delta f_i^{[t]}\|^2 + \underbrace{\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|^2}_{T_2}\notag\\
&\hspace{20pt}+\underbrace{\alpha_i^{[t]}\langle x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]}),\Delta f_i^{[t]}\rangle}_{T_3}+\underbrace{\langle x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]}),y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\rangle}_{T_4}\notag\\
&\hspace{20pt}+\underbrace{\alpha_i^{[t]}\langle\Delta f_i^{[t]},y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\rangle}_{T_5}.\label{lem:bound_x:proof_eq1}
\end{align}

We bound each term of \eqref{lem:bound_x:proof_eq1} separately. By the definition of $y_{i,k}$, we have
\begin{align*}
\widebar{F}_i(\{\theta_j^{[t]}\}_{j< i},\{y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\}_{k\geq i})=0.
\end{align*}
This implies
\begin{align}
&T_1\notag\\
&=\|x_i^{[t]}\|^2-2\alpha_i^{[t]}\langle x_i^{[t]},F_i(\vtheta^{[t]})\rangle+(\alpha_i^{[t]})^2\|F_i(\vtheta^{[t]})\|^2\notag\\
&=\|x_i^{[t]}\|^2\hspace{-2pt}-\hspace{-2pt}2\alpha_i^{[t]}\hspace{-2pt}\langle x_i^{[t]}\hspace{-2pt},\hspace{-2pt}\widebar{F}_i(\{\theta_j^{[t]}\}_{j\leq i},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k>i})\hspace{-2pt}-\hspace{-2pt}\widebar{F}_i(\{\theta_j^{[t]}\}_{j< i},\{y_{i,k}(\{\theta_j^{[t]}\}_{j<i})\}_{k\geq i})\rangle\notag\\
&\hspace{20pt}-2\alpha_i^{[t]}\langle x_i^{[t]}, \widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j\leq i},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k>i})\rangle+(\alpha_i^{[t]})^2\|\widebar{F}_i(\vtheta^{[t]})\|^2\notag\\
&=\|x_i^{[t]}\|^2-2\alpha_i^{[t]}\langle x_i^{[t]},\widebar{F}_i(\{\theta_j^{[t]}\}_{j\leq i},\theta_i^{[t]},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k>i})\notag\\
&\hspace{100pt}-\widebar{F}_i(\{\theta_j^{[t]}\}_{j< i},y_{i,i}(\{\theta_j^{[t]}\}_{j< i}),\{y_{i+1,k}(y_{i,i}(\{\theta_j^{[t]}\}_{j< i}),\{\theta_j^{[t]}\}_{j<i})\}_{k\geq i})\rangle\notag\\
&\hspace{20pt}-2\alpha_i^{[t]}\langle x_i^{[t]}, \widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j\leq i},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k>i})\rangle\notag\\
&\hspace{20pt}+(\alpha_i^{[t]})^2\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j< i},\{y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\}_{k\geq i})\|^2\notag\\
&\leq\|x_i^{[t]}\|^2-2\delta\alpha_i^{[t]}\|x_i^{[t]}\|^2+2\alpha_i^{[t]}\|x_i^{[t]}\|\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j\leq i},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k>i})\|\notag\\
&\hspace{20pt}+(\alpha_i^{[t]})^2\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j< i},\{y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\}_{k\geq i})\|^2\notag\\
&\leq\|x_i^{[t]}\|^2-2\delta\alpha_i^{[t]}\|x_i^{[t]}\|^2+\delta\alpha_i^{[t]}\|x_i^{[t]}\|^2+\frac{4N^3L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_{j}^{[t]}\|^2\notag\\
&\hspace{20pt}+4N^3 L^6(\alpha_i^{[t]})^2\sum_{j=i}^{N}\|x_j^{[t]}\|^2\notag\\
&= \|x_i^{[t]}\|^2-\left(\delta\alpha_i^{[t]}-4N^3L^6(\alpha_i^{[t]})^2\right)\|x_i^{[t]}\|^2+\left(\frac{4N^3L^6\alpha_i^{[t]}}{\delta}+4N^3 L^6(\alpha_i^{[t]})^2\right)\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2\notag\\
&\leq \|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{2}\|x_i^{[t]}\|^2+\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2,
\label{lem:bound_x:proof_eq2}
\end{align}
where the third equation follow from \eqref{eq:y_transformation}, the first inequality follows from Assumption~\ref{assump:stronglymonotone}, and the final inequality follows from the step size condition $\alpha_i^{[t]}\leq \frac{\delta}{8N^3 L^6}$ and $\alpha_i^{[t]}\leq \frac{1}{\delta}$.
% 
The second inequality uses the bound 
\[\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j\leq i},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k>i})\|\leq2NL^3\alpha_i^{[t]}\sum_{k=i+1}^{N}\|x_k^{[t]}\|,\] 
which we now justify
\begin{align}
&\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j\leq i},\{y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\}_{k>i})\|\notag\\
&\leq L\sum_{k=i+1}^{N}\|\theta_k^{[t]}-y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\|\notag\\
&\leq L\sum_{k=i+1}^{N}\|\theta_k^{[t]}-y_{k,k}(\{\theta_j^{[t]}\}_{j<k})\|^2+L\alpha_i^{[t]}\sum_{k=i+1}^{N}\|y_{k,k}(\{\theta_j^{[t]}\}_{j<k})-y_{i+1,k}(\{\theta_j^{[t]}\}_{j\leq i})\|\notag\\
&= L\sum_{k=i+1}^{N}\|x_k^{[t]}\|+L\alpha_i^{[t]}\sum_{k=i+1}^{N}\|y_{k,k}(\{\theta_j^{[t]}\}_{j<k})-y_{k,k}(\{\theta_j^{[t]}\}_{j\leq i},{y_{i,i'}(\{\theta_j^{[t]}\}_{j\leq i})}_{i'=i,\cdots,k-1})\|\notag\\
&\leq L\sum_{k=i+1}^{N}\|x_k^{[t]}\|+L^3\alpha_i^{[t]}\sum_{k=i+1}^{N}\sum_{j=i+1}^{k-1}\|x_j^{[t]}\|\notag\\
&\leq 2NL^3\sum_{k=i+1}^{N}\|x_k^{[t]}\|.
\label{lem:bound_x:proof_eq2.2}
\end{align}
The second inequality of \eqref{lem:bound_x:proof_eq2} plugs in the bound on $\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j< i},\{y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\}_{k\geq i})\|$ below, which follows from a similar argument
\begin{align*}
\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j< i},\{y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\}_{k\geq i})\|&\leq L\|x_i^{[t]}\|+L\sum_{k=i+1}^{N}\|\theta_k^{[t]}-y_{i,k}(\{\theta_j^{[t]}\}_{j<i})\|\notag\\
&\leq 2NL^3\sum_{k=i}^{N}\|x_k^{[t]}\|
\end{align*}




The term $T_2$ can be bounded leveraging the Lipschitz condition of $y_{i,i}$
\begin{align}
\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\| & \leq L\sum_{j=1}^{i-1}\|\theta_{j}^{[t+1]}-\theta_{j}^{[t]}\|\notag\\
&\leq L\sum_{j=1}^{i-1}\alpha_j^{[t]}\left(\|\Delta f_j^{[t]}\|+NL^2\sum_{k=j}^{N}\|x_k^{[t]}\|\right)\notag\\
&\leq L\sum_{j=1}^{i-1}\alpha_j^{[t]}\|\Delta f_j^{[t]}\|+N^2 L^3\sum_{j=1}^{i-1}\alpha_j^{[t]}\sum_{k=j}^{N}\|x_{k}^{[t]}\|,\label{lem:bound_x:proof_eq4.0}
\end{align}
where the second inequality plugs in the result of Lemma~\ref{lem:Lipschitz}.

Since $\alpha_j^{[t]}\leq\alpha_k^{[t]}$ for any $j\leq k$, ~\eqref{lem:bound_x:proof_eq4.0} implies
\begin{align}
T_2&= \|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|^2 \notag\\
% &\leq L^2\sum_{j=1}^{i-1}\|\theta_{j}^{[t+1]}-\theta_{j}^{[t]}\|^2\notag\\
% &\leq L^2\sum_{j=1}^{i-1}(\alpha_j^{[t]})^2\left(2\|\Delta f_j^{[t]}\|^2+2N^3 L^4\sum_{k=j}^{N}\|x_k^{[t]}\|^2\right)\notag\\
% &\leq 2L^2\sum_{j=1}^{i-1}(\alpha_j^{[t]})^2\|\Delta f_j^{[t]}\|^2+2N^4 L^6\sum_{j=1}^{N}(\alpha_j^{[t]})^2\|x_j^{[t]}\|^2.
&\leq 2\left(L\sum_{j=1}^{i-1}\alpha_j^{[t]}\|\Delta f_j^{[t]}\|\right)^2+2\left(N^2 L^3\sum_{j=1}^{N}\alpha_j^{[t]}\|x_{j}^{[t]}\|\right)^2\notag\\
&\leq 2NL^2\sum_{j=1}^{i-1}(\alpha_j^{[t]})^2\|\Delta f_j^{[t]}\|^2+2N^5 L^6\sum_{j=1}^{N}(\alpha_j^{[t]})^2\|x_{j}^{[t]}\|^2.
\label{lem:bound_x:proof_eq4}
\end{align}

Next we treat $T_3$
\begin{align}
T_3 &\leq \alpha_i^{[t]}\|\Delta f_i^{[t]}\|\|x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]})\|\notag\\
&\leq \frac{2\alpha_i^{[t]}}{\delta}\|\Delta f_i^{[t]}\|^2+\frac{\delta\alpha_i^{[t]}}{8}\|x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]})\|^2\notag\\
&\leq \frac{2\alpha_i^{[t]}}{\delta}\|\Delta f_i^{[t]}\|^2+\frac{\delta\alpha_i^{[t]}}{8}\left(\|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{2}\|x_i^{[t]}\|^2+\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2\right)\notag\\
&\leq \frac{2\alpha_i^{[t]}}{\delta}\|\Delta f_i^{[t]}\|^2+\frac{\delta\alpha_i^{[t]}}{8}\|x_i^{[t]}\|^2+\frac{N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2,
\end{align}
where the third inequality uses \eqref{lem:bound_x:proof_eq2} and the fourth inequality follows from the step size condition $\alpha_i^{[t]}\leq\frac{1}{\delta}$.

To bound $T_4$, we plug in \eqref{lem:bound_x:proof_eq2} and \eqref{lem:bound_x:proof_eq4.0}
\begin{align}
T_4&\leq \|x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]})\|\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|\notag\\
&\leq \sqrt{\|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{2}\|x_i^{[t]}\|^2+\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2}\quad\cdot\notag\\
&\hspace{50pt}\left(L\sum_{j=1}^{i-1}\alpha_j^{[t]}\|\Delta f_j^{[t]}\|+N L^3\sum_{j=1}^{i-1}\alpha_j^{[t]}\sum_{k=j}^{N}\|x_{k}^{[t]}\|\right)\notag\\
&\leq \left(\|x_i^{[t]}\|+\sqrt{\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}}\sum_{j=i+1}^{N}\|x_j^{[t]}\|\right)\cdot\notag\\
&\hspace{50pt}\left(L\sum_{j=1}^{i-1}\alpha_j^{[t]}\|\Delta f_j^{[t]}\|+N^2 L^3\sum_{j=1}^{i-1}\alpha_j^{[t]}\|x_{j}^{[t]}\|+N^2 L^3\alpha_{i-1}^{[t]}\sum_{j=i}^{N}\|x_{j}^{[t]}\|\right)\notag\\
&\leq L\sum_{j=1}^{i-1}\alpha_j^{[t]}\|\Delta f_j^{[t]}\|\|x_i^{[t]}\|+L^4(\alpha_i^{[t]})^{1/2}\alpha_{i-1}^{[t]}\sqrt{\frac{8N^3}{\delta}}\left(\sum_{j=i+1}^{N}\|x_j^{[t]}\|\right)\left(\sum_{j=1}^{i-1}\|\Delta f_j^{[t]}\|\right)\notag\\
&\hspace{20pt}+N^2 L^3\sum_{j=1}^{i-1}\alpha_j^{[t]}\|x_{j}^{[t]}\|\|x_i^{[t]}\|+N^2 L^3\alpha_{i-1}^{[t]} \sum_{j=i}^{N} \|x_{j}^{[t]}\| \|x_i^{[t]}\|\notag\\
&\hspace{20pt}+L^6(\alpha_i^{[t]})^{1/2}\alpha_{i-1}^{[t]}\sqrt{\frac{8N^7}{\delta}}\left(\sum_{j=i+1}^{N}\|x_j^{[t]}\|\right)\left(\sum_{j=1}^{N}\|x_j^{[t]}\|\right)\notag\\
&\leq \frac{NL\alpha_{i-1}^{[t]}}{4}\|x_i^{[t]}\|^2+L\sum_{j=1}^{i-1}\alpha_j^{[t]}\|\Delta f_j^{[t]}\|^2+NL^4(\alpha_i^{[t]})^{1/2}\alpha_{i-1}^{[t]}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+\frac{2N^4 L^4 (\alpha_i^{[t]})^{1/2}\alpha_{i-1}^{[t]}}{\delta}\sum_{j=i+1}^{N}\|\Delta f_j^{[t]}\|^2+\frac{4N^6 L^6\alpha_{i-1}^{[t]}}{\delta}\|x_i^{[t]}\|^2+\frac{\delta}{16N}\sum_{j=1}^{i-1}\alpha_{j}^{[t]}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+\frac{N^3 L^3\alpha_{i-1}^{[t]}}{4}\|x_i^{[t]}\|^2+N^2 L^3\alpha_{i-1}^{[t]}\sum_{j=i}^{N}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+NL^6(\alpha_i^{[t]})^{1/2}\alpha_{i-1}^{[t]}\sqrt{\frac{2N^7}{\delta}}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2+NL^6(\alpha_i^{[t]})^{1/2}\alpha_{i-1}^{[t]}\sqrt{\frac{2N^7}{\delta}}\sum_{j=1}^{N}\|x_j^{[t]}\|^2\notag\\
&\leq \sum_{j=1}^{i-1}\left(\frac{\delta\alpha_{j}^{[t]}}{16N}+NL^6\sqrt{\frac{2N^7}{\delta}}(\alpha_{i}^{[t]})^2\right)\|x_j^{[t]}\|^2+4N^2L^3\alpha_{i-1}^{[t]}\sum_{j=i}^{N}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+(\frac{N^3L^3\alpha_{i-1}^{[t]}}{2}+\frac{4N^6 L^6\alpha_{i-1}^{[t]}}{\delta})\|x_i^{[t]}\|^2+L\alpha_i^{[t]}\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2\notag\\
&\leq \sum_{j=1}^{i-1}\left(\frac{\delta\alpha_{j}^{[t]}}{16N}+NL^6\sqrt{\frac{2N^7}{\delta}}(\alpha_{i}^{[t]})^2\right)\|x_j^{[t]}\|^2+4N^2L^3\alpha_{i-1}^{[t]}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+(\frac{9N^3L^3\alpha_{i-1}^{[t]}}{2}+\frac{4N^6 L^6\alpha_{i-1}^{[t]}}{\delta})\|x_i^{[t]}\|^2+L\alpha_i^{[t]}\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2,
\end{align}
where the second inequality follows from the fact that $\sqrt{a_1+a_2+\cdots}\leq\sqrt{a_1}+\sqrt{a_2}+\cdots$ for any positive scalars $a_1,a_2,\cdots$. We have also simplified terms using the step size condition $\alpha_{i}^{[t]}\leq\frac{\delta}{2N^5 L^6}$, $\alpha_{i}^{[t]}\leq\frac{N^2}{L^2}$, and $\alpha_i^{[t]}\leq\frac{\delta^2}{4N^8 L^6}$.

We finally bound $T_5$ with \eqref{lem:bound_x:proof_eq4},
\begin{align}
T_5&\leq \alpha_i^{[t]}\|\Delta f_i^{[t]}\| \|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|\notag\\
&\leq (\alpha_i^{[t]})^2\|\Delta f_i^{[t]}\|^2+\frac{1}{4} \|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|^2\notag\\
&\leq (\alpha_i^{[t]})^2\|\Delta f_i^{[t]}\|^2+\frac{NL^2}{2}\sum_{j=1}^{i-1}(\alpha_j^{[t]})^2\|\Delta f_j^{[t]}\|^2+\frac{N^5 L^6}{2}\sum_{j=1}^{N}(\alpha_j^{[t]})^2\|x_{j}^{[t]}\|^2.
\end{align}

Collecting the bounds on $T_1$-$T_5$ and applying them to \eqref{lem:bound_x:proof_eq1}, we have
\allowdisplaybreaks
\begin{align*}
&\|x_i^{t+1}\|^2\notag\\
&\leq \|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{2}\|x_i^{[t]}\|^2+\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2+(\alpha_i^{[t]})^2\|\Delta f_i^{[t]}\|^2\notag\\
&\hspace{20pt}+2NL^2\sum_{j=1}^{i-1}(\alpha_j^{[t]})^2\|\Delta f_j^{[t]}\|^2+2N^5 L^6\sum_{j=1}^{N}(\alpha_j^{[t]})^2\|x_{j}^{[t]}\|^2\notag\\
&\hspace{20pt}+\frac{2\alpha_i^{[t]}}{\delta}\|\Delta f_i^{[t]}\|^2+\frac{\delta\alpha_i^{[t]}}{8}\|x_i^{[t]}\|^2+\frac{N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+\sum_{j=1}^{i-1}\left(\frac{\delta\alpha_{j}^{[t]}}{16N}+NL^6\sqrt{\frac{2N^7}{\delta}}(\alpha_{i}^{[t]})^2\right)\|x_j^{[t]}\|^2+4N^2L^3\alpha_{i-1}^{[t]}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+(\frac{9N^3L^3\alpha_{i-1}^{[t]}}{2}+\frac{4N^6 L^6\alpha_{i-1}^{[t]}}{\delta})\|x_i^{[t]}\|^2+L\alpha_i^{[t]}\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2\notag\\
&\hspace{20pt}+(\alpha_i^{[t]})^2\|\Delta f_i^{[t]}\|^2+\frac{NL^2}{2}\sum_{j=1}^{i-1}(\alpha_j^{[t]})^2\|\Delta f_j^{[t]}\|^2+\frac{N^5 L^6}{2}\sum_{j=1}^{N}(\alpha_j^{[t]})^2\|x_{j}^{[t]}\|^2\notag\\
&\leq \|x_i^{[t]}\|^2-\left(\frac{3\delta\alpha_i^{[t]}}{8}-\frac{9N^3L^3\alpha_{i-1}^{[t]}}{2}-\frac{4N^6 L^6\alpha_{i-1}^{[t]}}{\delta}+\frac{5N^5 L^6 (\alpha_i^{[t]})^2}{2}\right)\|x_i^{[t]}\|^2\notag\\
&\hspace{20pt}+\sum_{j=1}^{i-1}\left(\frac{5N^5 L^6 (\alpha_j^{[t]})^2}{2}+\frac{\delta\alpha_{j}^{[t]}}{16N}+NL^6\sqrt{\frac{2N^7}{\delta}}(\alpha_{i}^{[t]})^2\right)\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+\sum_{j=i+1}^{N}\left(\frac{9N^3 L^6\alpha_i^{[t]}}{\delta}+\frac{5N^5 L^6 (\alpha_j^{[t]})^2}{2}+4N^2 L^3\alpha_i^{[t]}\right)\|x_j^{[t]}\|^2+(\frac{3}{\delta}+L)\alpha_i^{[t]}\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2\notag\\
&\leq \|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{4}\|x_i^{[t]}\|^2+\sum_{j=1}^{i-1}\frac{\delta\alpha_j^{[t]}}{8N}\|x_j^{[t]}\|^2\notag\\
&\hspace{20pt}+\left(\frac{9N^3 L^6}{\delta}+8N^2 L^3\right)\alpha_i^{[t]}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2+(\frac{3}{\delta}+L)\alpha_i^{[t]}\sum_{j=1}^{N}\|\Delta f_j^{[t]}\|^2,
\end{align*}
where in the second inequality we have combined and simplified terms with the step size condition $\alpha_i^{[t]}\leq\frac{1}{\delta}$ and $\alpha_i^{[t]}\leq\frac{2}{5NL}$, and the third inequality follows from $\frac{\alpha_{i-1}^{[t]}}{\alpha_i^{[t]}}\leq\frac{\delta}{16}(\frac{9N^3 L^3}{2}+\frac{4N^6 L^6}{\delta})^{-1}$, $\alpha_i^{[t]}\leq\frac{\delta}{40N^5 L^6}$, $\frac{(\alpha_{i}^{[t]})^2}{\alpha_1^{[t]}}\leq\frac{\delta^{3/2}}{64N^7}$, $\alpha_i^{[t]}\leq\frac{\delta}{80N^6 L^6}$, and $\frac{(\alpha_{i}^{[t]})^2}{\alpha_1^{[t]}}\leq\frac{8}{5N^3 L^3}$.

\qed





\subsection{Proof of Lemma~\ref{lem:Lipschitz}}

By the definition of $f_i^{[t]}$,
\begin{align}
    \|f_i^{[t]}\|&=\|\Delta f_i^{[t]}+\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j<i},\{y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\}_{k\geq i})\|\notag\\
    &\leq\|\Delta f_i^{[t]}\|+\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\{\theta_j^{[t]}\}_{j<i},\{y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\}_{k\geq i})\|\notag\\
    &\leq\|\Delta f_i^{[t]}\|+L\sum_{k=i}^{N}\|\theta_k^{[t]}-y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\|.\label{lem:Lipschitz:proof_eq1}
\end{align}

Using the fact that $y_{i,k}(\{\theta_j'\}_{j<i})=y_{k,k}(\{\theta_j'\}_{j<i},\{y_{i,j}\}_{j=i,\cdots,k-1})$, we can bound the second term of \eqref{lem:Lipschitz:proof_eq1} recursively
\begin{align}
    &\sum_{k=i}^{N}\|\theta_k^{[t]}-y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\|\notag\\
    &\leq \|x_i^{[t]}\|+\sum_{k=i+1}^{N}\|\theta_k^{[t]}-y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\|\notag\\
    &\leq \|x_i^{[t]}\|+\|\theta_{i+1}^{[t]}-y_{i+1,i+1}(\{\theta_j^{[t]}\}_{j< i},y_{i,i}(\{\theta_j^{[t]}\}_{j< i}))\|+\sum_{k=i+2}^{N}\|\theta_k^{[t]}-y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\|\notag\\
    &\leq (L+1)\|x_i^{[t]}\|+\|x_{i+1}^{[t+1]}\|+\sum_{k=i+2}^{N}\|\theta_k^{[t]}-y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\|\notag\\
    &\leq (2L+1)\|x_i^{[t]}\|+(L+1)\|x_{i+1}^{[t]}\|+\|x_{i+2}^{[t]}\|+\sum_{k=i+3}^{N}\|\theta_k^{[t]}-y_{i,k}(\{\theta_j^{[t]}\}_{j< i})\|\notag\\
    &\leq NL\sum_{k=i}^{N}\|x_k^{[t]}\|.\label{lem:Lipschitz:proof_eq2}
\end{align}

Plugging \eqref{lem:Lipschitz:proof_eq2} into \eqref{lem:Lipschitz:proof_eq1}, we have
\begin{align}
    \|f_i^{[t]}\|\leq \|\Delta f_i^{[t]}\|+NL^2\sum_{k=i}^{N}\|x_k^{[t]}\|.\label{lem:Lipschitz:proof_eq3}
\end{align}

The bound on $\|\theta_i^{[t+1]}-\theta_i^{[t]}\|$ follows simply from \eqref{lem:Lipschitz:proof_eq3} and the update rule \eqref{alg:update_decision}.


\qed


\subsection{Proof of Lemma~\ref{lem:conv_x_standardSA}}
\label{sec:proof_lem:conv_x_standardSA}

By the update rule \eqref{alg:update_standardSA}, we have
\begin{align*}
x_i^{[t+1]}&=\theta_{i}^{[t+1]}-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\notag\\
&=\theta_{i}^{[t]}-\alpha_i^{[t]}F_i(\vtheta^{[t]},X^{[t]})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\notag\\
&=x_i^{[t]}-\alpha_i^{[t]}F_i(\vtheta^{[t]},X^{[t]})+\left(y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\right)\notag\\
&=x_i^{[t]}-\alpha_i^{[t]} \widebar{F}_i(\vtheta^{[t]})\hspace{-2pt}-\hspace{-2pt}\alpha_i^{[t]}\big(F_i(\vtheta^{[t]},X^{[t]})\hspace{-2pt}-\hspace{-2pt}\widebar{F}_i(\vtheta^{[t]})\big)\hspace{-2pt}+\hspace{-2pt}\big(y_{i,i}(\{\theta_j^{[t]}\}_{j<i})\hspace{-2pt}-\hspace{-2pt}y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\big).
\end{align*}

Taking the norm,
\begin{align}
&\|x_i^{[t+1]}\|^2\notag\\
&=\underbrace{\|x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]})\|^2}_{A_1}+\underbrace{(\alpha_i^{[t]})^2\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2}_{A_2}\notag\\
&\hspace{20pt}+\underbrace{\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|^2}_{A_3}+\underbrace{\alpha_i^{[t]}\langle x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]}),F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle}_{A_4}\notag\\
&\hspace{20pt}+\underbrace{\langle x_i^{[t]}-\alpha_i^{[t]}\widebar{F}_i(\vtheta^{[t]}),y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\rangle}_{A_5}\notag\\
&\hspace{20pt}+\underbrace{\alpha_i^{[t]}\langle F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]}), y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})}_{A_6}\rangle.
\label{lem:conv_x_standardSA_proof_eq1}
\end{align}

A bound on $A_1$ can be obtained using an argument identical to \eqref{lem:bound_x:proof_eq2}, provided that the step sizes satisfy $\alpha_i^{[t]}\leq \frac{\delta}{8N^3 L^6}$ and $\alpha_i^{[t]}\leq \frac{1}{\delta}$
\begin{align}
A_1&=\|x_i^{[t]}\|^2-2\alpha_i^{[t]}\langle x_i^{[t]},\widebar{F}_i(\vtheta^{[t]})\rangle+(\alpha_i^{[t]})^2\|\widebar{F}_i(\vtheta^{[t]})\|^2\notag\\
&\leq \|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{2}\|x_i^{[t]}\|^2+\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2.
% &= \|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{2}\|x_i^{[t]}\|^2+\frac{216 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{3}\|x_j^{[t]}\|^2.
\label{lem:conv_x_standardSA_proof_eq2}
\end{align}

% The second term is bounded in expectation due to Assumption~\ref{assump:noise_bounded}
% \begin{align}
% \mathbb{E}[A_2]=\mathbb{E}_{X^{[t]}\sim\xi}[(\alpha_i^{[t]})^2\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2]\leq B(\alpha_i^{[t]})^2.\label{lem:conv_x_standardSA_proof_eq3}
% \end{align}


The second term is bounded in expectation due to Assumption~\ref{assump:bounded}
\begin{align}
A_2=(\alpha_i^{[t]})^2\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|^2\leq 4D^2(\alpha_i^{[t]})^2.\label{lem:conv_x_standardSA_proof_eq3}
\end{align}

Using the Lipschitz continuity of $y_{i,i}$, we have
\begin{align}
\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|& \leq L\sum_{j=1}^{i-1}\|\theta_{j}^{[t+1]}-\theta_{j}^{[t]}\|\notag\\
&= L\sum_{j=1}^{i-1}\alpha_j^{[t]}\|F_i(\vtheta^{[t]},X^{[t]})\|\notag\\
&\leq NLD\alpha_{i-1}^{[t]},\label{lem:conv_x_standardSA_proof_eq4}
\end{align}
which implies
\begin{align}
A_3&= \|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|^2 \leq N^2 L^2 D^2 (\alpha_{i-1}^{[t]})^2.
\label{lem:conv_x_standardSA_proof_eq5}
\end{align}

The term $A_4$ is obviously zero in expectation as
\begin{align*}
\mathbb{E}[F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})]=0.
\end{align*}

The bound on $A_5$ follows from the Cauchy-Schwarz inequality
\begin{align}
A_5&\leq\|x_i^{[t]}\|\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|\notag\\
&\hspace{20pt}+\alpha_i^{[t]}\|\widebar{F}_i(\vtheta^{[t]})\|\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|\notag\\
&\leq \frac{\delta\alpha_i^{[t]}}{4}\|x_i^{[t]}\|^2+\frac{1}{\delta\alpha_i^{[t]}}\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|^2\notag\\
&\hspace{20pt}+D\alpha_i^{[t]}\|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|\notag\\
&\leq \frac{\delta\alpha_i^{[t]}}{4}\|x_i^{[t]}\|^2+\frac{(NLD\alpha_{i-1}^{[t]})^2}{\delta\alpha_i^{[t]}}+D\alpha_i^{[t]}\cdot NLD\alpha_{i-1}^{[t]}\notag\\
&\leq \frac{\delta\alpha_i^{[t]}}{4}\|x_i^{[t]}\|^2+\frac{N^2 L^2 D^2 (\alpha_{i-1}^{[t]})^2}{\delta\alpha_i^{[t]}}+ NLD^2\alpha_i^{[t]}\alpha_{i-1}^{[t]}
\label{lem:conv_x_standardSA_proof_eq7}
\end{align}
where in the third equality we plug in \eqref{lem:conv_x_standardSA_proof_eq4}.

Finally, we bound $A_6$ using a similar argument
\begin{align}
A_6&\leq \alpha_i^{[t]}\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\| \|y_{i,i}(\{\theta_j^{[t]}\}_{j<i})-y_{i,i}(\{\theta_j^{[t+1]}\}_{j<i})\|\notag\\
&\leq \alpha_i^{[t]}\cdot 2D\cdot NLD\alpha_{i-1}^{[t]}\notag\\
&\leq  2 NLD^2\alpha_{i-1}^{[t]}\alpha_i^{[t]}.
\label{lem:conv_x_standardSA_proof_eq8}
\end{align}

Collecting the bounds in \eqref{lem:conv_x_standardSA_proof_eq2}-\eqref{lem:conv_x_standardSA_proof_eq8} and putting them into \eqref{lem:conv_x_standardSA_proof_eq1}, we get
\begin{align*}
&\mathbb{E}[\|x_i^{[t+1]}\|^2]\\
&\leq \mathbb{E}[\|x_i^{[t]}\|^2-\frac{\delta\alpha_i^{[t]}}{2}\|x_i^{[t]}\|^2+\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\|x_j^{[t]}\|^2+4D^2(\alpha_i^{[t]})^2+N^2 L^2 D^2 (\alpha_{i-1}^{[t]})^2\notag\\
&\hspace{20pt}+\frac{\delta\alpha_i^{[t]}}{4}\|x_i^{[t]}\|^2+\frac{N^2 L^2 D^2 (\alpha_{i-1}^{[t]})^2}{\delta\alpha_i^{[t]}}+ NLD^2\alpha_i^{[t]}\alpha_{i-1}^{[t]}+2 NLD^2\alpha_{i-1}^{[t]}\alpha_i^{[t]}]\notag\\
&\leq \mathbb{E}[\|x_i^{[t]}\|^2]-\frac{\delta\alpha_i^{[t]}}{4}\mathbb{E}[\|x_i^{[t]}\|^2]+\frac{8N^3 L^6\alpha_i^{[t]}}{\delta}\sum_{j=i+1}^{N}\mathbb{E}[\|x_j^{[t]}\|^2]\notag\\
&\hspace{20pt}+8N^2 L^2 D^2 (\alpha_{i}^{[t]})^2+\frac{N^2 L^2 D^2 (\alpha_{i-1}^{[t]})^2}{\delta\alpha_i^{[t]}}.
\end{align*}

\qed



\subsection{Proof of Lemma~\ref{lem:Markovian_crossterm}}

% We introduce an auxiliary Markov chain $\{\widetilde{X}^{[t]}\}$ generated under the decision variable $\vtheta^{[t-\tau_t]}$ starting from $X^{[t-\tau_t]}$ as follows
% \begin{align}
% {X}^{[t-\tau_t]} \stackrel{\vtheta^{[t-\tau_t]}}{\longrightarrow}  \widetilde{X}^{[t-\tau_t+1]} \stackrel{\vtheta^{[t-\tau_t]}}{\longrightarrow}  \cdots \widetilde{X}^{[k-1]} \stackrel{\vtheta^{[t-\tau_t]}}{\longrightarrow}  \widetilde{X}^{[k]}.
% \label{eq:def_distribution_d}
% \end{align}
% Let $\widetilde{\mu}$ denote the stationary distribution of this Markov chain.
% We recall how the original time-varying Markov chain $\{X^{[t]}\}$ is generated
% \begin{align*}
% X^{[t-\tau_t]} \stackrel{\vtheta^{[t-\tau_t+1]}}{\longrightarrow} X^{[t-\tau_t+1]}  \stackrel{\vtheta^{[t-\tau_t+2]}}{\longrightarrow} \cdots \stackrel{\vtheta^{[t-1]}}{\longrightarrow} X^{[t-1]} \stackrel{\vtheta^{[k]}}{\longrightarrow} X^{[k]}.
% \end{align*}


% We decompose $\mathbb{E}[\langle\Delta f_i^{[t]},F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle]=T_1+T_2+T_3+T_4$,
% where
% \begin{align*}
%     &T_1 = \mathbb{E}[\langle \Delta f_i^{[t]}-\Delta f_i^{[t-\tau_t]},F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\rangle]\notag\\
%     &T_2 = \mathbb{E}[\langle \Delta f_i^{[t-\tau_t]},F_i(\vtheta^{[t]},X^{[t]})-F_i(\vtheta^{[t]},\widetilde{X}^{[t]})\rangle]\notag\\
%     &T_3 = \mathbb{E}[\langle \Delta f_i^{[t-\tau_t]}, F_i(\vtheta^{[t]},\widetilde{X}^{[t]})-\mathbb{E}_{X\sim\widetilde{\mu}}[F_i(\vtheta^{[t]},X)]\rangle]\notag\\
%     &T_4 = \mathbb{E}[\langle \Delta f_i^{[t-\tau_t]}, \mathbb{E}_{X\sim\widetilde{\mu}}[F_i(\vtheta^{[t]},X)]-\widebar{F}_i(\vtheta^{[t]})\rangle].
% \end{align*}

% We treat each term separately. First, by the definition of $\Delta f_i^{[t]}$ in \eqref{eq:residuals}
% \begin{align*}
% T_1&\leq\mathbb{E}[\| \Delta f_i^{[t]}- \Delta f_i^{[t-\tau_t]}\|\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|]\notag\\
% &\leq \mathbb{E}[\|f_i^{[t]}- f_i^{[t-\tau_t]}\|\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|]\notag\\
% &\hspace{20pt}+\mathbb{E}[\|\widebar{F}_i(\vtheta^{[t]})-\widebar{F}_i(\vtheta^{[t-\tau_t]})\|\|F_i(\vtheta^{[t]},X^{[t]})-\widebar{F}_i(\vtheta^{[t]})\|]\notag\\
% &\leq \mathbb{E}\left[2\Big((NB+1)L+L\sum_{j=1}^{N}\|x_j^{[t]}\|\Big)\sum_{t'=0}^{\tau_t-1}\|f_i^{[t-t']}-f_i^{[t-t'-1]}\|\right]\notag\\
% &\hspace{20pt}+ \mathbb{E}\left[2\Big((NB+1)L+L\sum_{j=1}^{N}\|x_j^{[t]}\|\Big)\right]\notag\\
% &\leq 2\lambda^{[t-\tau_t]}
% \end{align*}
% where the third inequality follows from \eqref{lem:bound_Deltaf:boundedF}

% \qed

This lemma essentially bounds the distance between samples from a time-varying Markov chain and the stationary distribution. Techniques for proving this lemma has been well-studied in the literature. Hence we omit the proof here but note that it is very similar to the proof of Lemma 1 in \citet{zeng2024two}.
